Synthetic Image Oversampling for Rare-Class Representation Learning in Deep Facial Phenotyping

Recent deep facial phenotyping methods can support the recognition of genetic syndromes, but patient images are often scarce and unevenly distributed across disorders. Synthetic facial images offer a way to supplement the training data without collecting additional patient photographs. Their usefulness, however, depends on whether they improve recognition of real patients: generated images may introduce artifacts or repeat features already represented in the training set. It is therefore necessary to examine both how much synthetic augmentation to use and which disorders benefit. We investigate disease-specific synthetic oversampling using images from the Phenotypic Disease Image Database to augment a subset of the GestaltMatcher Database. We compare increasing augmentation levels in an image-based model, GestaltMatcher-Arc, and a multimodal model, GestaltMML, while keeping the real training and patient-disjoint evaluation partitions fixed. Repeated training runs assess overall and disease-specific accuracy, and an exploratory embedding analysis examines changes in class compactness and separation. Augmentation improves mean recognition accuracy in both training setups, although gains remain modest in GestaltMatcher-Arc and continue across the tested levels in GestaltMML. These aggregate improvements are accompanied by uneven disease-level responses, including reduced accuracy for some disorders. In the embedding analysis, disorders with fewer real training images tend to gain more class separation, but geometric changes do not consistently track classification performance. Together, the findings support synthetic oversampling for limited-data facial phenotyping and emphasize the need to assess its amount and benefit for individual disorders within each training setup.

==> liao_manuscript/1abstract.tex <==

Recent deep facial phenotyping methods can support the recognition of genetic syndromes, but patient images are often scarce and unevenly distributed across disorders. Synthetic facial images offer a way to supplement the training data without collecting additional patient photographs. Their usefulness, however, depends on whether they improve recognition of real patients: generated images may introduce artifacts or repeat features already represented in the training set. It is therefore necessary to examine both how much synthetic augmentation to use and which disorders benefit. We investigate disease-specific synthetic oversampling using images from the Phenotypic Disease Image Database to augment a subset of the GestaltMatcher Database. We compare increasing augmentation levels in an image-based model, GestaltMatcher-Arc, and a multimodal model, GestaltMML, while keeping the real training and patient-disjoint evaluation partitions fixed. Repeated training runs assess overall and disease-specific accuracy, and an exploratory embedding analysis examines changes in class compactness and separation. Augmentation improves mean recognition accuracy in both training setups, although gains remain modest in GestaltMatcher-Arc and continue across the tested levels in GestaltMML. These aggregate improvements are accompanied by uneven disease-level responses, including reduced accuracy for some disorders. In the embedding analysis, disorders with fewer real training images tend to gain more class separation, but geometric changes do not consistently track classification performance. Together, the findings support synthetic oversampling for limited-data facial phenotyping and emphasize the need to assess its amount and benefit for individual disorders within each training setup.

==> liao_manuscript/4methods.tex <==
\section{Methods}
\label{sec:methods}
\subsection{Study Design and Dataset}

We used a curated subset of the GestaltMatcher Database (GMDB v1.1.0)
\citep{lesmann2024gestaltmatcher} containing 1,847 real facial images from
10 genetic disorders. A fixed patient-disjoint partition assigned 1,289
images to training and 558 images to evaluation, corresponding to an
approximately 70\%/30\% split. Training counts ranged from 312 images for
Cornelia de Lange syndrome to 41 images for 22q11.2 deletion syndrome,
giving a largest-to-smallest class ratio of 7.6. The real-data partitions
were identical across models, augmentation conditions, and training seeds.
Synthetic images were added only to training. Figure~\ref{fig:workflow}
summarizes the study design.

To screen for potential overlap between synthetic training images and the real evaluation partition, we compared the full synthetic pool against all evaluation images using exact pixel-level hashes, perceptual hashes, and nearest-neighbor cosine similarity in the 512-dimensional GestaltMatcher-Arc embedding space. Embedding similarities were calibrated against real-training-to-evaluation nearest-neighbor similarities.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.90\textwidth]
    {liao_manuscript/figures/figure1_experimental_workflow.pdf}
    \caption{Study design. A patient-disjoint GMDB partition contains
    1,289 real training images and 558 real evaluation images. Nested
    PDIDB subsets augment the training data under PD25, PD50, PD75,
    and PD100. GestaltMatcher-Arc and GestaltMML are trained with three
    seeds per condition. The real partitions and synthetic subsets are
    fixed across training seeds.}
    \label{fig:workflow}
\end{figure*}

\subsection{Synthetic Image Augmentation}

We obtained synthetic facial images from the Phenotype Diseased Image
Synthesis Database (PDIDB) \citep{pdidb}, generated with our
disease-conditioned StyleGAN3 model \citep{Karras2021}. We defined five experimental conditions. 
Baseline used only
real training images. PD25, PD50, PD75, and PD100 added approximately
25\%, 50\%, 75\%, and 100\% of each disorder's available synthetic pool,
respectively. These percentages refer to the synthetic pool, not to the
size of the real training set.


The synthetic subsets were sampled once using random seed 11 and nested across augmentation conditions. These subsets were held fixed across all model-training runs, so the three training seeds did not change which synthetic images were included.
Table~\ref{tab:dataset_composition} reports
the real and synthetic image counts. The augmented conditions added 433,
866, 1,298, and 1,727 images, producing total training sets of 1,722,
2,155, 2,587, and 3,016 images. Figure~\ref{fig:synthetic_examples} shows
examples from the disorders with the fewest real training images.

\begin{table}[t]
    \centering
    \caption{Dataset composition. Train and Eval. are the fixed,
    patient-disjoint real-image partitions. The Baseline condition consists of the real training images only,  while PD25–PD100 indicate the numbers of synthetic images added under the four augmentation conditions.}
    \label{tab:dataset_composition}
    \small
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{lrrrrrr}
        \toprule
        \textbf{Disorder} &
        \textbf{Train} &
        \textbf{Eval.} &
        \textbf{PD25} &
        \textbf{PD50} &
        \textbf{PD75} &
        \textbf{PD100} \\
        \midrule
        Cornelia de Lange     & 312 & 135 & 46 & 91 & 137 & 182 \\
        Williams-Beuren       & 191 & 82  & 47 & 93 & 140 & 186 \\
        Noonan                & 145 & 62  & 48 & 95 & 143 & 190 \\
        Kabuki                & 144 & 62  & 40 & 81 & 121 & 161 \\
        KBG                   & 125 & 54  & 47 & 94 & 140 & 187 \\
        Angelman              & 111 & 49  & 42 & 85 & 127 & 169 \\
        Rubinstein-Taybi      & 81  & 35  & 44 & 89 & 133 & 177 \\
        Smith-Magenis         & 71  & 31  & 42 & 83 & 125 & 166 \\
        Nicolaides-Baraitser  & 68  & 29  & 42 & 84 & 126 & 168 \\
        22q11.2 deletion      & 41  & 19  & 35 & 71 & 106 & 141 \\
        \midrule
        \textbf{Total} &
        \textbf{1,289} &
        \textbf{558} &
        \textbf{433} &
        \textbf{866} &
        \textbf{1,298} &
        \textbf{1,727} \\
        \bottomrule
    \end{tabular}
\end{table}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.82\textwidth]
    {liao_manuscript/figures/figure2_representative_synthetic_images.pdf}
    \caption{PDIDB synthetic facial images. Two examples are shown for
    each of the five disorders with the fewest real training images.
    Synthetic images are used only for training.}
    \label{fig:synthetic_examples}
\end{figure*}

\subsection{Model Training}
\label{sec:model_training}
Both models were trained under all five conditions using three model-training random seeds (11, 22, and 33) on NVIDIA A100 GPUs. These seeds controlled training stochasticity, including random parameter initialization and data shuffling, while the real-data partitions and synthetic subsets remained unchanged.

\subsubsection{GestaltMatcher-Arc}

GestaltMatcher-Arc \citep{hustinx2023improving} uses a ResNet-50 face
backbone pretrained on Glint360K \citep{an2021partial} with ArcFace loss
\citep{deng2019arcface}. We froze the convolutional backbone and trained
the 512-dimensional feature projection and 10-class classifier for
50 epochs. Training used Adam optimizer with a batch size of 64 and learning rates
of $5\times10^{-4}$ for the projection layer and $10^{-3}$ for the classifier.
A ReduceLROnPlateau scheduler used a reduction factor of 0.5 and patience
of five epochs.

We used class-frequency-weighted cross-entropy with class weight
\begin{equation}
    w_c = 0.5 + 0.5\frac{n_{\min}}{n_c},
    \label{eq:class_weight}
\end{equation}
where $n_c$ denotes the training count for class $c$ and $n_{\min}$ is
the smallest class count. Synthetic oversampling was thus evaluated
together with loss weighting. To assess whether the augmentation effect depended on class-frequency weighting, we repeated the Baseline and PD50 conditions across all three seeds using unweighted cross-entropy as an ablation study.


\subsubsection{GestaltMML}

We initialized GestaltMML \citep{wu2024gestaltmml} from
\texttt{dandelin/vilt-b32-mlm} \citep{kim2021vilt} and used a 10-class
output head. Each real training image formed two image-text pairs.
One contained clinical text with sex, age, ethnicity, and Human Phenotype
Ontology (HPO) terms; the other used the placeholder token ``*''.
Each synthetic image formed one pair with the placeholder because
corresponding clinical metadata were unavailable. This construction
produced 2,578, 3,011, 3,444, 3,876, and 4,305 training pairs for
Baseline, PD25, PD50, PD75, and PD100, respectively.

We fine-tuned the model for 10 epochs using AdamW with a
learning rate of $5\times10^{-5}$, a batch size of 64, and a maximum
text length of 40.
% Specify the clinical-text input used during evaluation.

\subsection{Classification Evaluation}
\label{sec:metric_definition}

For each training run, we selected the checkpoint with the highest overall Top-1 accuracy on the real-image evaluation partition, breaking ties in favor of the earliest epoch. The same partition was used to report classification performance.


Let $N$ be the number of evaluation images, $C=10$ the number of classes,
and $N_c$ the number of evaluation images in class $c$. For image $i$,
$y_i$ is the true label and $\hat{y}_i$ is the predicted label. Overall
Top-1 accuracy weights images equally:
\begin{equation}
    \mathrm{Top1}
    = \frac{1}{N}\sum_{i=1}^{N}\mathbf{1}(\hat{y}_i=y_i).
    \label{eq:top1}
\end{equation}
Mean per-class Top-1 accuracy weights classes equally:
\begin{equation}
    \mathrm{MeanTop1}
    = \frac{1}{C}\sum_{c=1}^{C}
      \frac{1}{N_c}\sum_{i:y_i=c}\mathbf{1}(\hat{y}_i=c).
    \label{eq:mean_top1}
\end{equation}
We also report Top-3 and Top-5 accuracy, defined by whether the true
label appears among the three or five highest-ranked predictions.

Classification metrics are reported as mean and sample standard
deviation across the three training seeds. For disease-specific
comparisons, we calculated the percentage-point difference from
Baseline within each seed and then summarized these paired differences
across seeds.

\subsection{Embedding Analysis}

We conducted an exploratory analysis of GestaltMatcher-Arc embeddings
using the seed-11 Baseline and PD50 runs. PD50 was selected after
examining classification results because it had the highest mean
overall Top-1 accuracy across training seeds. Both runs were analyzed
on the same real evaluation images using their $L_2$-normalized,
512-dimensional embeddings.

Global class structure was summarized by the mean cosine-distance
silhouette score \citep{rousseeuw1987silhouettes}. For image $i$,
\begin{equation}
    s(i) = \frac{b(i)-a(i)}{\max\{a(i),b(i)\}},
    \label{eq:silhouette}
\end{equation}
where $a(i)$ is the mean cosine distance to other images in the same
class. For each other class, we calculated the mean cosine distance
from image $i$ to that class; $b(i)$ is the smallest of these means.

We additionally calculated three disease-level measures. Compactness
is the mean cosine distance between a class's embeddings and its
$L_2$-normalized centroid. Nearest-centroid separation is the cosine
distance from that centroid to the closest centroid of another class.
The separation-to-compactness ratio divides separation by compactness.
Lower compactness indicates tighter clusters, while higher separation
indicates greater distance between class centroids. All quantitative
measures were calculated in the original embedding space. PCA and UMAP
were used only for visualization.

\subsection{Statistical Analysis}

For each embedding metric $M$, we calculated the relative change from
Baseline to PD50 as
\begin{equation}
    \Delta M(\%)
    = 100\frac{M_{\mathrm{PD50}}-M_{\mathrm{Baseline}}}
    {M_{\mathrm{Baseline}}}.
    \label{eq:relative_change}
\end{equation}
We used Spearman rank correlation with two-sided $p$-values to assess
associations between real training class size and relative changes in
each metric. These analyses involved 10 disorders and a single training
seed and were interpreted as exploratory associations.

==> liao_manuscript/5results.tex <==
\section{Experiments}
\label{sec:experiments}

We evaluate how the amount of synthetic augmentation affects recognition
accuracy in two training setups. We first compare overall and per-class
performance, then examine representation changes and their association
with the number of real training images per disorder.



\subsection{Experimental Setup}

We compare GestaltMatcher-Arc and GestaltMML across Baseline and four nested synthetic augmentation conditions (PD25--PD100), using the fixed patient-disjoint partition described in Section~\ref{sec:methods}. Each condition was trained with seeds 11, 22, and 33. We compare augmentation effects within each model because their architectures and training procedures differ.

\subsection{Overall Classification Performance}

Figure~\ref{fig:overall_performance} compares overall and mean per-class
Top-1 accuracy across augmentation conditions. Both models achieved
higher mean overall Top-1 accuracy with synthetic augmentation than at
Baseline, but their responses to additional synthetic images differed.

For GestaltMatcher-Arc, mean overall Top-1 accuracy increased from
$89.19\pm0.92\%$ at Baseline to its highest observed value of
$90.20\pm0.58\%$ at PD50. Differences among augmented conditions were
small relative to the variation across training seeds. Mean per-class
Top-1 accuracy instead peaked at PD25, reaching $89.15\pm0.80\%$ compared
with $87.23\pm1.18\%$ at Baseline. Thus, the condition with the highest
overall accuracy differed from the condition with the highest mean
per-class accuracy. 

To assess sensitivity to class-frequency weighting, we repeated the Arc Baseline and PD50 conditions using unweighted cross-entropy (Table~\ref{tab:class_weight_ablation}). The paired PD50 gain was $+1.02 \pm 1.72$ percentage points without weighting, compared with $+1.02 \pm 1.49$ points with weighting. These almost identical mean gains suggest that the observed augmentation effect did not depend strongly on class-frequency weighting.

For GestaltMML, mean overall Top-1 accuracy increased across the tested
augmentation levels, from $68.82\pm1.53\%$ at Baseline to
$74.31\pm0.90\%$ at PD100. Mean per-class Top-1 accuracy also increased,
from $64.02\pm2.14\%$ to $69.39\pm1.03\%$. Complete Top-1, mean per-class
Top-1, Top-3, and Top-5 results are reported in
Table~\ref{tab:overall_results} in the appendix.

% The original manuscript reports a paired gain of 5.50 percentage points.
% Verify this value against unrounded per-seed results before reinstating it.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.92\textwidth]
    {liao_manuscript/figures/figure3_overall_performance_multiseed.pdf}
    \caption{Classification accuracy across augmentation conditions.
    Bars show mean overall and mean per-class Top-1 accuracy across
    three training seeds; error bars show one sample standard deviation.
    Checkpoints are selected and evaluated on the same fixed real-image
    partition.}
    \label{fig:overall_performance}
\end{figure*}

\subsection{Disease-Specific Performance}

Figure~\ref{fig:disease_heatmaps} reports paired changes in disease-specific
Top-1 accuracy from Baseline, calculated within each training seed and
then averaged across seeds. For GestaltMatcher-Arc, higher mean overall
accuracy did not imply improvement for every disorder; disease-specific
changes varied across augmentation conditions and training seeds.

At PD100, GestaltMML improved mean Top-1 accuracy for seven disorders.
The largest paired gains occurred for KBG ($+16.05$ percentage points),
Williams-Beuren ($+14.63$), and Smith-Magenis ($+12.90$). Mean accuracy
also increased for Noonan ($+5.91$), 22q11.2 deletion ($+5.26$),
Nicolaides-Baraitser ($+2.30$), and Cornelia de Lange ($+2.22$).
In contrast, mean accuracy decreased for Rubinstein-Taybi
($-3.81$ percentage points), Kabuki ($-1.08$), and Angelman ($-0.68$).
The improvement in aggregate performance therefore included both gains
and losses at the disease level.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.90\textwidth]
    {liao_manuscript/figures/figure4_disease_specific_heatmaps_multiseed.pdf}
    \caption{Disease-specific changes in Top-1 accuracy from Baseline.
    Values are mean $\pm$ sample standard deviation of paired
    percentage-point differences across three training seeds. Each
    difference is calculated against the Baseline run with the same seed.
    Disorders are ordered by real training image count, from largest
    to smallest.}
    \label{fig:disease_heatmaps}
\end{figure*}

\subsection{Embedding-Space Analysis}

We compared Baseline and PD50 embeddings from the seed-11
GestaltMatcher-Arc runs using the same 558 real evaluation images.
PD50 was selected because it achieved the highest mean overall Top-1
accuracy across seeds; this analysis is exploratory. The mean
cosine-distance silhouette score increased from 0.228 at Baseline to
0.267 at PD50. This corresponds to a relative increase of 16.9\%,
calculated from unrounded values.

Nearest-centroid separation increased for nine of the ten disorders
(Table~\ref{tab:embedding_results}). The largest relative increases were
observed for Smith-Magenis and 22q11.2 deletion (both $+23.91\%$),
followed by KBG ($+18.56\%$) and Angelman ($+18.46\%$). Cornelia de Lange
was the only disorder with reduced separation ($-9.86\%$).

Compactness improved for eight disorders. Mean distance to the class
centroid increased slightly for Smith-Magenis ($+2.35\%$) and 22q11.2
deletion ($+0.94\%$), even though their nearest-centroid separation
increased. The separation-to-compactness ratio increased for nine
disorders and decreased for Cornelia de Lange ($-0.56\%$). These results
show that compactness and separation can change differently under the
same augmentation condition.

Figure~\ref{fig:arc_umap} shows a shared UMAP projection of the Baseline
and PD50 representations. Quantitative results are calculated in the
original embedding space.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.88\textwidth]
    {liao_manuscript/figures/figure5a_arc_umap_baseline_vs_pd50.pdf}
    \caption{Shared UMAP projection of seed-11 GestaltMatcher-Arc
    embeddings at Baseline and PD50. Each point represents one of the
    same 558 real evaluation images; colors indicate disorder.
    Quantitative metrics use the original $L_2$-normalized,
    512-dimensional embeddings.}
    \label{fig:arc_umap}
\end{figure*}

\subsection{Association With Real Training Class Size}

Across the ten disorders, real training class size was inversely
associated with relative change in nearest-centroid separation
(Spearman $\rho=-0.707$, $p=0.022$). Disorders with fewer real training
images tended to show larger relative separation gains at PD50 in
this seed-11 analysis.

The corresponding correlations were $\rho=0.527$ ($p=0.117$) for
relative compactness change and $\rho=-0.588$ ($p=0.074$) for relative
change in the separation-to-compactness ratio. These exploratory
associations describe variation across disorders in one training run;
they do not establish that smaller class size causes a greater benefit
from augmentation.

\subsection{Discussion}

The two training setups respond differently to additional synthetic
images. GestaltMatcher-Arc shows modest gains with little variation
among augmented conditions, while GestaltMML continues to improve
across the tested levels. Their backbones, trainable parameters,
optimization, and input construction differ, so this comparison does
not identify which component accounts for the different responses.
The results support assessing augmentation amount within each training
setup rather than assuming that the same amount is suitable for both.

The class-size association suggests that limited real training data
may be relevant to changes in representation geometry. However, this
association concerns centroid separation, not a direct measure of
recognition benefit. Cornelia de Lange improves in mean classification
accuracy under some augmentation conditions while its separation
decreases in the seed-11 PD50 analysis. Disease-level accuracy and
single-seed geometry therefore provide different summaries of the
augmentation response. The geometric results alone cannot explain
accuracy changes across repeated training runs.

The evaluation covers ten disorders, one synthetic image source,
and one patient partition. Repeated training seeds capture training
variability but do not assess uncertainty from alternative patient
partitions or synthetic subsets. The representation analysis uses
one seed and a condition selected after examining classification
results, limiting the conclusions that can be drawn from its
cross-disease associations. Checkpoint selection and performance
reporting also use the same evaluation partition, so the reported
accuracies are not independent test estimates. The findings concern
recognition on this benchmark; clinical utility has not been established.

==> liao_manuscript/6discussion.tex <==
% \section{Discussion}

% Synthetic oversampling improved mean performance across three training seeds
% for both models, but they responded differently: GestaltMatcher-Arc showed
% relatively small differences across augmentation levels, whereas GestaltMML
% showed a stronger dose-dependent improvement through PD100. The models differ
% in backbone training (frozen ResNet-50 versus fully fine-tuned ViLT),
% optimization, and input construction, so we report this contrast as an
% empirical finding rather than attribute it to any single factor.

% Disease-level results suggest that data scarcity may contribute to augmentation
% benefit, and lower-data classes tended to gain more nearest-centroid separation
% in the representative GestaltMatcher-Arc embedding analysis
% ($\rho=-0.707$). Responses were heterogeneous across diseases and training
% seeds, however, so scarcity is unlikely to be the sole determinant. The
% largest class, Cornelia de Lange syndrome, also showed improved mean
% classification performance under some augmentation conditions, while its
% nearest-centroid separation decreased by 9.86\% in the representative
% seed-11 PD50 embedding analysis, suggesting that changes in classification
% performance and representation geometry did not necessarily occur in parallel.

==> liao_manuscript/7future.tex <==
% \section{Limitations and Future Directions}

% We evaluated ten disorders, one synthetic-image source, and one fixed
% patient-disjoint partition without an external cohort. Although each condition
% was evaluated across three training seeds, these repeated runs capture training
% variability but not uncertainty arising from alternative patient partitions or
% synthetic subset compositions. The size--separation association rests solely
% on ten classes. Natural next steps are evaluation across additional patient
% partitions and synthetic subsets, additional generators, substantially rarer
% disorders, external validation, and controlled ablations separating backbone,
% optimization, and input design. For the multimodal model, Shapley-based
% cross-modal attribution such as \textit{MultiSHAP}~\citep{multishap} could
% further clarify whether augmentation gains arise from the facial images, the
% clinical text, or their interaction. Improved accuracy and embedding separation
% on this benchmark do not establish clinical utility, and the models are research
% tools rather than diagnostic systems.

==> liao_manuscript/tables/datasetcomposition.tex <==
\begin{table}[h]
\centering
\caption{
Composition of the 10-disorder GMDB subset and synthetic augmentation
conditions. Real Train and Eval. denote the fixed patient-disjoint real-image
partitions. PD25--PD100 report the number of synthetic images added to the
training set for each disease.
}
\label{tab:dataset_composition}
\small
\setlength{\tabcolsep}{4.5pt}
\begin{tabular}{lrrrrrr}
\toprule
\textbf{Disease} &
\textbf{Train} &
\textbf{Eval.} &
\textbf{PD25} &
\textbf{PD50} &
\textbf{PD75} &
\textbf{PD100} \\
\midrule
Cornelia de Lange      & 312 & 135 & 46 & 91 & 137 & 182 \\
Williams--Beuren       & 191 & 82  & 47 & 93 & 140 & 186 \\
Noonan                  & 145 & 62  & 48 & 95 & 143 & 190 \\
Kabuki                  & 144 & 62  & 40 & 81 & 121 & 161 \\
KBG                     & 125 & 54  & 47 & 94 & 140 & 187 \\
Angelman                & 111 & 49  & 42 & 85 & 127 & 169 \\
Rubinstein--Taybi      & 81  & 35  & 44 & 89 & 133 & 177 \\
Smith--Magenis         & 71  & 31  & 42 & 83 & 125 & 166 \\
Nicolaides--Baraitser  & 68  & 29  & 42 & 84 & 126 & 168 \\
22q11.2 deletion       & 41  & 19  & 35 & 71 & 106 & 141 \\
\midrule
\textbf{Total} &
\textbf{1,289} &
\textbf{558} &
\textbf{433} &
\textbf{866} &
\textbf{1,298} &
\textbf{1,727} \\
\bottomrule
\end{tabular}
\end{table}
